A Linearized L1-Galerkin FEM for Non-smooth Solutions of Kirchhoff type Quasilinear Time-fractional Integro-differential Equation

In this article, we study the semi discrete and fully discrete formulations for a Kirchhoff type quasilinear integro-differential equation involving time-fractional derivative of order $\alpha \in (0,1) $. For the semi discrete formulation of the equation under consideration, we discretize the space domain using a conforming FEM and keep the time variable continuous. We modify the standard Ritz-Volterra projection operator to carry out error analysis for the semi discrete formulation of the considered equation. In general, solutions of the time-fractional partial differential equations (PDEs) have a weak singularity near time $t=0$. Taking this singularity into account, we develop a new linearized fully discrete numerical scheme for the considered equation on a graded mesh in time. We derive a priori bounds on the solution of this fully discrete numerical scheme using a new weighted $H^{1}(\Omega)$ norm. We prove that the developed numerical scheme has an accuracy rate of $O(P^{-1}+N^{-(2-\alpha)})$ in $L^{\infty}(0,T;L^{2}(\Omega))$ as well as in $L^{\infty}(0,T;H^{1}_{0}(\Omega))$, where $P$ and $N$ are degrees of freedom in the space and time directions respectively. The robustness and efficiency of the proposed numerical scheme are demonstrated by some numerical examples.

==> 8_revision.tex <==
\newpage
\noindent Professor Chi-Wang Shu\\
Editor-in-Chief\\
Journal of Scientific Computing\\

\noindent Dear Prof. Shu
\par  First of all, we would like to thank the editor-in-chief and two referees for their valuable comments and constructive suggestions that have helped us to improve this work.
\par We have revised the manuscript in the light of their suggestions. We believe that we have addressed all  concerns raised by the editor-in-chief and referees in the revised version of the manuscript. We have made all changes in \textcolor{blue}{blue} colour in the revised manuscript. We hope that the revised manuscript is now suitable for publication in the Journal of Scientific Computing. 
\par The point-wise responses to the comments of the editor-in-chief and two referees regarding our manuscript entitled \emph{"A Linearized FEM for Non-smooth Solutions of
Kirchhoff type Quasilinear Time-fractional Integro-differential Equation"} are given below.
\subsection{Response to the comment of editor-in-chief}
\textbf{Comment:}~Include a numerical test problem with variable memory operator. \\
\textbf{Response:}~We have added a test problem as Example 5.2 where we have taken the memory operator with variable coefficients. 
\subsection{ Responses to the comments of Reviewer 1}
\textbf{Comment-1:}~It is true that some time-fractional equations have a weak singularity near $t=0$. In order to obtain  an optimal grading parameter, the regularity of the exact solution  should be given. Could you please show some references related to the exact solution or proved by yourselves?\\

\noindent \textbf{Response-1:}~In \cite{huang2020optimal}, Huang $et. al.$ studied  the following linear  time-fractional initial boundary value problem     
 \begin{equation} \label{22-8-22-1-1}
\begin{aligned}
^{C}\mathcal{D}^{\alpha}_{t}u-\Delta u&=f(x,t)\quad \text{in}~ \Omega \times (0,T],\\
u(x,0)&=u_{0}(x) \quad \text{in} ~\Omega,\\
u&=0 \quad \text{in}~\partial \Omega \times (0,T].
\end{aligned}
\end{equation}
\noindent Let $\{(\lambda_{i},\phi_{i}), i=1,2,\dots\}$ be the eigenvalues and eigenfunctions for the boundary value problem  $-\Delta \phi_{i}=\lambda_{i}\phi_{i}~~ \text{in}~~ \Omega $ with homogeneous Dirichlet boundary condition. The eigenfunctions are normalised by taking $\|\phi_{i}\|=1$ for all $i$. From the theory of sectorial operator \cite{henry2006geometric} the fractional power $\Delta^{\mu}$ of the operator $\Delta$ is defined for each $\mu \in \mathbb{R}$ with domain 
\begin{equation*}
D(\Delta^{\mu})=\{g \in  L^{2}(\Omega);~ \sum_{j=1}^{\infty}\lambda_{j}^{2\mu}~|(g,\phi_{j})|^{2} < \infty\},
\end{equation*}
and the norm is given by 
\begin{equation*}
    \|g\|^{2}_{\Delta^{\mu}}= \sum_{j=1}^{\infty}\lambda_{j}^{2\mu}~|(g,\phi_{j})|^{2}.
\end{equation*}
\noindent For example $D(\Delta^{1/2})=H^{1}_{0}(\Omega)$ and $D(\Delta)=H^{2}(\Omega)\cap H^{1}_{0}(\Omega)$.
They have proved the following regularity on the solution of \eqref{22-8-22-1-1}.
\begin{lem} \cite{huang2020optimal}
Let $q \in \mathbb{N}\cup \{0\}$. Assume that $u_{0}\in D(\Delta^{q+2})$ and $\partial^{l}_{t}f(\cdot,t)\in D(\Delta^{q})$ for $t\in (0,T]$ and that $\|u_{0}\|_{\Delta^{q+2}}+\|\partial^{l}_{t}f(\cdot,t)\|_{\Delta^{q+1}} \lesssim C$ for $l=1,2$. Then the solution of \eqref{22-8-22-1-1} satisfies 
\begin{align}
\|u(\cdot,t)\|_{q}& \lesssim C,~\forall~ t \in (0,T]\label{14-9-22-1-1}\\
\|\partial^{l}_{t}u(\cdot,t)\|_{q} &\lesssim C(1+t^{\alpha-l})~~l=0,1,2,3,~\forall ~t \in (0,T]\label{14-9-22-2-1}\\
\|~^{C}\mathcal{D}^{\alpha}_{t}u(\cdot,t)\|_{q}& \lesssim C~\forall~ t \in (0,T]. \label{14-9-22-3-1}
\end{align}
\end{lem}
\noindent In this work, we derive semidiscrete and fully discrete error estimates under the assumption that the solution $u$ of our considered equation satisfies \eqref{14-9-22-1-1}-\eqref{14-9-22-3-1}. We could not prove these estimates \eqref{14-9-22-1-1}-\eqref{14-9-22-3-1}  yet. This is definitely  an interesting and challenging task which require further investigations.\\

\noindent \textbf{Comment-2:}~In the numerical results, the case for $\alpha=0.4,0.5,0.6$ are presented. What about the convergence behaviour for smaller or larger values of $\alpha$. Will these case reach $2-\alpha$ order convergence with the grading parameter showed in this work?\\

\noindent \textbf{Response-2:}~ 

\newpage
\subsection{Reviewer-2}
\textbf{Q-1}\quad $M$ is used to denote the degrees of freedom in space. In page 2 the nonlocal diffusion coefficient also denoted by $M$. One has to use different notations here. \\

\noindent \textbf{Ans-1} We have changed the notation for degrees of freedom in the space direction from $M$ to $P$. Now it is different from the notation of diffusion coefficient.\\

\noindent \textbf{Q-2} \quad In page 10, the last term in the RHS is not correct. We only have $B(t,s,\rho,\tilde{g})=(b\rho,\tilde{g})\neq (\rho,b\tilde{g})$. Arguments below this inequality need to be correct.\\

\noindent \textbf{Q-3}\quad Page 13, Line 53, The notation of discrete Laplacian operator should be denoted differently from the usual Laplace operator $\Delta$.\\

\noindent \textbf{Ans-3}  We have changed the notation of discrete Laplacian operator from usual Laplacain as $\Delta_{h}$.

\noindent \textbf{Q-4} \quad Result (3.34) in  Theorem 3.4 needs to be reproved when taking $v_{h}=\Delta_{h}\theta$ in (3.36) how can you  prove the last term in RHS?
\begin{equation}
    B(t,s,\theta,\Delta_{h}\theta) \leq B_{0}\|\nabla \theta \|^{2}
\end{equation}
\noindent \textbf{Q-5} \quad This same mistake is repeated in the proof of Theorem 4.6 when taking the test function by $-\Delta_{h}u_{h}^{1}$ which means (4.24) does not hold.\\

\noindent \textbf{Q-6} \quad As a consequence the proof of uniqueness $u_{h}^{1}$ in Theorem 4.8 is incorrect when approximate solution don't satisfies (4.24).\\

\noindent \textbf{Q-7} \quad Page no 20, Notations in line 56,57 are confusing, Since $u^{n}=u(t_{n})$ is defined as a ffunction of $x$. What does it mean $u_{t}^{n}$ and $u_{tt}^{n}.$\\

\noindent \textbf{Ans-7} we have corrected the notations of $u_{tt}^{n}$.

\noindent \textbf{Q-8}\quad Page no 28, the example 5.1 in the numerical implementation section is a simple particular case of the equation in which $b_{2}=1, b_{1}=b_{0}=0$,The proof of theorems 3.2 and 4.6 is only true when these are constants functions. Perhapse numerial simulations are coincided with the theoretical results because of the special example with constant coefficients.  


